Constellation: A High Performance Geo-Distributed Middlebox Framework

Middleboxes are increasingly deployed across geographically distributed data centers. In these scenarios, the WAN latency between different sites can significantly impact the performance of stateful middleboxes. The deployment of middleboxes across such infrastructures can even become impractical due to the high cost of remote state accesses. We introduce Constellation, a framework for the geo distributed deployment of middleboxes. Constellation uses asynchronous replication of specialized state objects to achieve high performance and scalability. The evaluation of our implementation shows that, compared with the state-of-the-art [80], Constellation improves the throughput by a factor of 96 in wide area networks.

==> config.tex <==
\usepackage{usenix2019_v3}
\usepackage{filecontents}
\usepackage{amsmath}
\usepackage{mathtools}
\usepackage{cite}
\usepackage[english]{babel}
\usepackage{amssymb}
\usepackage{pifont}
\usepackage{textcomp}
\usepackage{tikz}
\usepackage{graphicx}
\usepackage{arydshln}
\usepackage{mathrsfs}
\usepackage{wasysym}
\usepackage{algorithm}
\usepackage{algorithmicx}
\usepackage{algpseudocode}
\usepackage{comment}
\usepackage[utf8]{inputenc}
\usepackage{multirow}
\usepackage{cleveref}
\usepackage{enumitem}
\usepackage{setspace}
\usepackage{url}
\usepackage{xspace}
\usepackage{accents}
\usepackage{ragged2e}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{nth}
\usepackage{tightheaders}
\usepackage{blindtext}
\usepackage{booktabs} % For formal tables
\usepackage{outlines}
\usepackage{color}

\newcommand{\fig}[1]{Figure~\ref{fig:#1}}
\newcommand{\tabl}[1]{Table~\ref{table:#1}}
\newcommand{\alg}[1]{Algorithm~\ref{algorithm:#1}}

\newcommand{\sect}[1]{\S~\ref{section:#1}}
\newcommand{\eqn}[1]{Eq.~\ref{equation:#1}}
\newcommand{\inv}[1]{Invariant~\ref{invariant:#1}}

\newcommand{\red}{}
\newcommand{\blue}{}

\let\emptyset\varnothing

